Benchmarking the Non-flow Contributions to the Elliptic Flow Parameter ($v_{_2}$) in Proton-Proton Collisions

This manuscript reports on the elliptic flow parameter, $v_{_2}$, in proton-proton (p-p) collisions using PYTHIA8 event generator simulations. The typical Event Plane ($EP$) method $v_{_2}$($EP$) as the one used for the real data analysis has been adopted to measure the $v_{_2}$ of particles composed of different quark flavors, and produced at mid-pseudorapidity $|\eta| \le 1$ at center-of-mass energy $\sqrt{s}$ = 200 GeV and $\sqrt{s}$ = 13 TeV. The event plane has been constructed using the soft charged particles with transverse momentum ($p{_{_T}} < $ 2 GeV/c) produced in various $\eta$ ranges. The pseudorapidity gap technique ($\Delta\eta$) between the particle of interest and the soft charged particles contributed to the event plane constructions has been utilized to benchmark the non-flow contributions. The $v_{_2}^{\pi^{^\pm,}\pi^{^0}}$, $v_{_2}^{J/\psi,\Upsilon, K, D, B}$, and the $v_{_2}^{\gamma_{dir}}$ show similar pattern dependence on the transverse momentum for the same $\Delta\eta$, at both $\sqrt{s}$ = 200 GeV and $\sqrt{s}$ = 13 TeV. At each center-of-mass energy, the measured $v_{_2}$ shows obvious dependence on the quark flavor contents where $v_{_2}^{\gamma_{dir}}$ $\le$ $v_{_2}^{J/\psi, \Upsilon, K, D, B}$ $\le$ $v_{_2}^{\pi^{^\pm,}\pi^{^0}}$ for similar $\Delta\eta$ gap. The measured $v_{_2}$ shows slightly higher values at smaller $\sqrt{s}$ for particles of similar values of $\Delta\eta$ gaps, particularly at small $\Delta\eta$ gap. The measured $v_{_2}$ for all particles shows systematic decreases with increasing the $\Delta\eta$ gap as expected from the previous experimental results. Because PYTHIA8 simulations do not incorporate final state interactions, the $v_{_2}(EP)$ values reported here primarily reflect the non-flow contributions and its dependence on the quark contents, pseudorapidity gap as a function on $p_{T}$ at each center of mass-energy.

==> bibliography.tex <==
%%%%%%%%%%%%%%%Introduction%%%%%%%%
@article{lim2019examination,
  title={Examination of flow and nonflow factorization methods in small collision systems},
  author={Lim, SH and Hu, Q and Belmont, R and Hill, KK and Nagle, JL and Perepelitsa, DV},
  journal={Physical Review C},
  volume={100},
  number={2},
  pages={024908},
  year={2019},
  publisher={APS}
}

@article{schenke2011flow,
  title={Flow in heavy-ion collisions—theory perspective},
  author={Schenke, Bj{\"o}rn},
  journal={Journal of Physics G: Nuclear and Particle Physics},
  volume={38},
  number={12},
  pages={124009},
  year={2011},
  publisher={IOP Publishing}
}


@article{luzum2011flow,
  title={Flow fluctuations and long-range correlations: elliptic flow and beyond},
  author={Luzum, Matthew},
  journal={Journal of Physics G: Nuclear and Particle Physics},
  volume={38},
  number={12},
  pages={124026},
  year={2011},
  publisher={IOP Publishing}
}


@article{voloshin1996flow,
  title={Flow study in relativistic nuclear collisions by Fourier expansion of azimuthal particle distributions},
  author={Voloshin, S and Zhang, Y},
  journal={Zeitschrift f{\"u}r Physik C Particles and Fields},
  volume={70},
  pages={665--671},
  year={1996},
  publisher={Springer}
}

@book{puri2020advances,
  title={Advances in Nuclear Physics: Structure and Reactions},
  author={Puri, Rajeev K and Aichelin, Joerg and Gautam, Sakshi and Kumar, Rohit},
  volume={257},
  year={2020},
  publisher={Springer Nature}
}

@incollection{teaney2010viscous,
  title={Viscous hydrodynamics and the quark gluon plasma},
  author={Teaney, Derek A},
  booktitle={Quark-Gluon Plasma 4},
  pages={207--266},
  year={2010},
  publisher={World Scientific}
}

@incollection{kolb2004hydrodynamic,
  title={Hydrodynamic description of ultrarelativistic heavy-ion collisions},
  author={Kolb, Peter F and Heinz, Ulrich},
  booktitle={Quark--Gluon Plasma 3},
  pages={634--714},
  year={2004},
  publisher={World Scientific}
}

@article{adil2006eccentricity,
  title={Eccentricity in heavy-ion collisions from color glass condensate initial conditions},
  author={Adil, Azfar and Drescher, Hans-Joachim and Dumitru, Adrian and Hayashigaki, Arata and Nara, Yasushi},
  journal={Physical Review C},
  volume={74},
  number={4},
  pages={044905},
  year={2006},
  publisher={APS}
}

@article{snellings2011elliptic,
  title={Elliptic flow: a brief review},
  author={Snellings, Raimond},
  journal={New Journal of Physics},
  volume={13},
  number={5},
  pages={055008},
  year={2011},
  publisher={IOP Publishing}
}

%%%%%%%%Literature Review%%%%%%%%
@article{trogolo2021directed,
  title={Directed, elliptic and triangular flow of D mesons in ALICE},
  author={Trogolo, Stefano},
  journal={PoS},
  pages={071},
  year={2021},
  publisher={SISSA}
}

@techreport{hu2020production,
  title={Production and azimuthal anisotropy of muons from heavy flavor decays in small and large systems with ATLAS},
  author={Hu, Qipeng},
  year={2020},
  institution={ATL-COM-PHYS-2020-403}
}

@article{acharya2018d,
  title={D-Meson Azimuthal Anisotropy in Midcentral Pb-Pb Collisions at $\sqrt{sNN}=5.02$ \text{TeV}},
  author={Acharya, Shreyasi and Adamov{\'a}, Dagmar and Adolfsson, Jonatan and Aggarwal, Madan M and Rinella, G Aglieri and Agnello, Michelangelo and Agrawal, Nikita and Ahammed, Zubayer and Ahmad, Nazeer and Ahn, Sang Un and others},
  journal={Physical review letters},
  volume={120},
  number={10},
  pages={102301},
  year={2018},
  publisher={APS}
}

@article{sjostrand2015introduction,
  title={An introduction to PYTHIA 8.2},
  author={Sj{\"o}strand, Torbj{\"o}rn and Ask, Stefan and Christiansen, Jesper R and Corke, Richard and Desai, Nishita and Ilten, Philip and Mrenna, Stephen and Prestel, Stefan and Rasmussen, Christine O and Skands, Peter Z},
  journal={Computer physics communications},
  volume={191},
  pages={159--177},
  year={2015},
  publisher={Elsevier}
}

@article{abelev2013d,
  title={D meson elliptic flow in noncentral Pb-Pb collisions at s N N= 2.76 TeV},
  author={Abelev, Betty and Adam, J and Adamov{\'a}, D and Adare, AM and Aggarwal, MM and Rinella, G Aglieri and Agnello, Michelangelo and Agocs, AG and Agostinelli, A and Ahammed, Z and others},
  journal={Physical review letters},
  volume={111},
  number={10},
  pages={102301},
  year={2013},
  publisher={APS}
}

@article{chatterjee2006elliptic,
  title={Elliptic flow of thermal photons in relativistic nuclear collisions},
  author={Chatterjee, Rupa and Frodermann, Evan S and Heinz, Ulrich and Srivastava, Dinesh K},
  journal={Physical review letters},
  volume={96},
  number={20},
  pages={202302},
  year={2006},
  publisher={APS}
}

@article{ollitrault1992anisotropy,
  title={Anisotropy as a signature of transverse collective flow},
  author={Ollitrault, Jean-Yves},
  journal={Physical Review D},
  volume={46},
  number={1},
  pages={229},
  year={1992},
  publisher={APS}
}

@article{bozek2011elliptic,
  title={Elliptic flow in proton--proton collisions at},
  author={Bozek, Piotr},
  journal={Eur. Phys. J. C},
  volume={71},
  pages={1530},
  year={2011},
  publisher={Springer}
}

@article{bautista2009particle,
  title={Particle production azimuthal asymmetries in a clustering of color sources model},
  author={Bautista, I and Cunqueiro, L and de Deus, J Dias and Pajares, C},
  journal={Journal of Physics G: Nuclear and Particle Physics},
  volume={37},
  number={1},
  pages={015103},
  year={2009},
  publisher={IOP Publishing}
}

@article{luzum2009viscous,
  title={Viscous hydrodynamic predictions for nuclear collisions at the LHC},
  author={Luzum, Matthew and Romatschke, Paul},
  journal={Physical review letters},
  volume={103},
  number={26},
  pages={262302},
  year={2009},
  publisher={APS}
}

@article{cunqueiro2010nuclear,
  title={Nuclear-like effects in proton--proton collisions at high energy},
  author={Cunqueiro, L and Dias de Deus, J and Pajares, C},
  journal={The European Physical Journal C},
  volume={65},
  pages={423--426},
  year={2010},
  publisher={Springer}
}

@article{zhu2005elliptic,
  title={Elliptic flow analysis in Au+ Au collisions at s NN= 200 GeV: Fluctuations vs non-flow effects},
  author={Zhu, Xianglei and Bleicher, Marcus and St{\"o}cker, Horst},
  journal={Physical Review C},
  volume={72},
  number={6},
  pages={064911},
  year={2005},
  publisher={APS}
}

@article{li2010re,
  title={Re-Examination for the Calculation of Elliptic Flow and Other Fourier Harmonics},
  author={Li, Xiao-Mei and Dong, Bao-Guo and Yan, Yu-Liang and Ma, Hai-Liang and Zhou, Dai-Mei and Sa, Ben-Hao},
  journal={Modern Physics Letters A},
  volume={25},
  number={14},
  pages={1211--1217},
  year={2010},
  publisher={World Scientific}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@article{shuryak2002azimuthal,
  title={Azimuthal asymmetry at large p t seem to be too large for a pure “jet quenching”},
  author={Shuryak, EV},
  journal={Physical Review C},
  volume={66},
  number={2},
  pages={027902},
  year={2002},
  publisher={APS}
}

@book{simili2008elliptic,
  title={Elliptic flow measurement at alice},
  author={Simili, Emanuele Lorenzo},
  year={2008},
  publisher={Utrecht University}
}


@article{zakharov2004radiative,
  title={Radiative parton energy loss and jet quenching in high-energy heavy-ion collisions},
  author={Zakharov, Bronislav Glebovich},
  journal={Journal of Experimental and Theoretical Physics Letters},
  volume={80},
  number={10},
  pages={617--622},
  year={2004},
  publisher={Springer}
}

@article{fries2003high,
  title={High-energy photons from passage of jets through quark-gluon plasma},
  author={Fries, Rainer J and M{\"u}ller, Berndt and Srivastava, Dinesh K},
  journal={Physical review letters},
  volume={90},
  number={13},
  pages={132301},
  year={2003},
  publisher={APS}
}

@article{turbide2006azimuthal,
  title={Azimuthal asymmetry of direct photons in high energy nuclear collisions},
  author={Turbide, Simon and Gale, Charles and Fries, Rainer J},
  journal={Physical review letters},
  volume={96},
  number={3},
  pages={032303},
  year={2006},
  publisher={APS}
}

@article{barrette1997proton,
  title={Proton and pion production relative to the reaction plane in Au+Au collisions at 11 A GeV/c},
  author={Barrette, Ji and Bellwied, R and Bennett, S and Bersch, R and Braun-Munzinger, P and Chang, WC and Cleland, WE and Clemen, M and Cole, J and Cormier, TM and others},
  journal={Physical Review C},
  volume={56},
  number={6},
  pages={3254},
  year={1997},
  publisher={APS}
}%%%%%%%%%%%%%%%%%

@article{alfiky2020onset,
  title={Onset of the jet quenching phenomenon},
  author={AlFiky, Mohamed T and Elsherif, Olfat and Hamed, Ahmed M},
  journal={JETP Letters},
  volume={111},
  number={1},
  pages={8--17},
  year={2020},
  publisher={Springer}
}

@article{adams2005experimental,
  title={Experimental and theoretical challenges in the search for the quark--gluon plasma: The STAR Collaboration's critical assessment of the evidence from RHIC collisions},
  author={Adams, John and Aggarwal, MM and Ahammed, Z and Amonett, J and Anderson, BD and Arkhipkin, D and Averichev, GS and Badyal, SK and Bai, Y and Balewski, J and others},
  journal={Nuclear Physics A},
  volume={757},
  number={1-2},
  pages={102--183},
  year={2005},
  publisher={Elsevier}
}

@article{adams2004azimuthal,
  title={Azimuthal Anisotropy and Correlations at Large Transverse Momenta in p+p and Au+A u Collisions at $\sqrt{sNN}=200$ \text{GeV}},
  author={Adams, John and Aggarwal, MM and Ahammed, Z and Amonett, J and Anderson, BD and Arkhipkin, D and Averichev, GS and Badyal, SK and Bai, Y and Balewski, J and others},
  journal={Physical review letters},
  volume={93},
  number={25},
  pages={252301},
  year={2004},
  publisher={APS}
}

@article{adare2010azimuthal,
  title={Azimuthal Anisotropy of $\pi^0$  Production in Au+ Au Collisions at $\sqrt{sNN}= 200$ \text{GeV}: Path-Length Dependence of Jet Quenching and the Role of Initial Geometry},
  author={Adare, Andrew and Afanasiev, S and Aidala, C and Ajitanand, NN and Akiba, Y and Al-Bataineh, H and Alexander, J and Aoki, K and Aramaki, Y and Atomssa, ET and others},
  journal={Physical review letters},
  volume={105},
  number={14},
  pages={142301},
  year={2010},
  publisher={APS}
}

@article{abelev2010parton,
  title={Parton energy loss in heavy-ion collisions via direct-photon and charged-particle azimuthal correlations},
  author={Abelev, BI and Aggarwal, MM and Ahammed, Z and Alakhverdyants, AV and Anderson, BD and Arkhipkin, D and Averichev, GS and Balewski, J and Barannikova, O and Barnby, LS and others},
  journal={Physical Review C},
  volume={82},
  number={3},
  pages={034909},
  year={2010},
  publisher={APS}
}

@article{adler2005centrality,
  title={Centrality dependence of direct photon production in $\sqrt{sNN}=200$ \text{GeV Au+Au} collisions},
  author={Adler, Stephen Scott and Afanasiev, S and Aidala, C and Ajitanand, NN and Akiba, Y and Alexander, J and Amirikas, R and Aphecetche, Laurent and Aronson, SH and Averbeck, R and others},
  journal={Physical review letters},
  volume={94},
  number={23},
  pages={232301},
  year={2005},
  publisher={APS}
}

@article{beddo2003star,
  title={The STAR barrel electromagnetic calorimeter},
  author={Beddo, M and Bielick, E and Fornek, T and Guarino, V and Hill, D and Krueger, K and LeCompte, T and Lopiano, D and Spinka, H and Underwood, D and others},
  journal={Nuclear Instruments and Methods in Physics Research Section A: Accelerators, Spectrometers, Detectors and Associated Equipment},
  volume={499},
  number={2-3},
  pages={725--739},
  year={2003},
  publisher={Elsevier}
}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@article{abelev2008centrality,
  title={Centrality dependence of charged hadron and strange hadron elliptic flow from $\sqrt{sNN}=200$ \text{GeV Au+Au} collisions},
  author={Abelev, BI and Aggarwal, MM and Ahammed, Z and Anderson, BD and Arkhipkin, D and Averichev, GS and Bai, Y and Balewski, J and Barannikova, O and Barnby, LS and others},
  journal={Physical Review C},
  volume={77},
  number={5},
  pages={054901},
  year={2008},
  publisher={APS}
}%%%%%%%%%%%%%%%%%%%%%%%%%%%%%flo2

@article{poskanzer1998methods,
  title={Methods for analyzing anisotropic flow in relativistic nuclear collisions},
  author={Poskanzer, Arthur M and Voloshin, Sergei A},
  journal={Physical Review C},
  volume={58},
  number={3},
  pages={1671},
  year={1998},
  publisher={APS}
}%%%%%%%%%%%%%%%%%%%%%%%%%flow2

@article{kasmaei2020photon,
  title={Photon production and elliptic flow from a momentum-anisotropic quark-gluon plasma},
  author={Kasmaei, Babak S and Strickland, Michael},
  journal={Physical Review D},
  volume={102},
  number={1},
  pages={014037},
  year={2020},
  publisher={APS}
}
